Prompt-Aware Controllable Shadow Removal

Shadow removal aims to restore the image content in shadowed regions. While deep learning-based methods have shown promising results, they still face key challenges: 1) uncontrolled removal of all shadows, or 2) controllable removal but heavily relies on precise shadow region masks. To address these issues, we introduce a novel paradigm: prompt-aware controllable shadow removal. Unlike existing approaches, our paradigm allows for targeted shadow removal from specific subjects based on user prompts (e.g., dots, lines, or subject masks). This approach eliminates the need for shadow annotations and offers flexible, user-controlled shadow removal. Specifically, we propose an end-to-end learnable model, the Prompt-Aware Controllable Shadow Removal Network (PACSRNet). PACSRNet consists of two key modules: a prompt-aware module that generates shadow masks for the specified subject based on the user prompt, and a shadow removal module that uses the shadow prior from the first module to restore the content in the shadowed regions. Additionally, we enhance the shadow removal module by incorporating feature information from the prompt-aware module through a linear operation, providing prompt-guided support for shadow removal. Recognizing that existing shadow removal datasets lack diverse user prompts, we contribute a new dataset specifically designed for prompt-based controllable shadow removal. Extensive experimental results demonstrate the effectiveness and superiority of PACSRNet.

==> tables/tab2.tex <==
\begin{table*}[t!]
% \centering\setlength{\tabcolsep}{3.5pt}
\tabcolsep 6pt
\renewcommand\arraystretch{1.1}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l||c|c|c|c|c|c|c|c|c}
\hline\thickhline
\rowcolor[HTML]{f8f9fa} & \multicolumn{3}{c|}{Shadow Regions} & \multicolumn{3}{c|}{Non-Shadow Regions} & \multicolumn{3}{c}{All Regions} \\ \cline{2-10}
% \cmidrule{2-10}
\rowcolor[HTML]{f8f9fa} \multirow{-2}{*}{Method}  & PSNR$\uparrow$ &  SSIM$\uparrow$ &   RMSE$\downarrow$ & PSNR$\uparrow$ &  SSIM$\uparrow$ &   RMSE$\downarrow$ & PSNR$\uparrow$ &  SSIM$\uparrow$ &   RMSE$\downarrow$ \\ \hline
% \multicolumn{5}{@{}p{6.8cm}}{\small{Consistency regularzation}} \\ \midrule
%Input Image & 20.83 & 0.930 & 39.01 & 37.46 & 0.985 & 2.40 & 20.46 & 0.894 & 8.40 \\
BMNet~\cite{zhu2022bijective} & 37.87 & 0.991 & 5.62 & 37.51 & 0.985 & 2.45 & 33.98 & 0.972 & 2.97 \\
%SG-ShadowNet~\cite{wan2022style} & 36.80 & 0.990 & 5.93 & 35.57 & 0.978 & 2.92 & 32.46 & 0.962 & 3.41 \\
Inpaint4Shadow~\cite{li2023leveraging} & 38.10 & 0.990 & 6.09 & 37.66 & 0.981 & 2.82 & 34.16 & 0.967 & 3.35 \\ 
ShadowFormer~\cite{guo2023shadowformer} & 39.48 & \underline{0.992} & 5.23 & 38.82 & 0.983 & 2.30 & 35.46 & 0.971 & 2.78 \\
ShadowDiffusion~\cite{guo2023shadowdiffusion} & \underline{39.69} & \underline{0.992} & 4.97 & 38.89 & \textbf{0.987} & 2.28 & \underline{35.67} & \textbf{0.975} & 2.72 \\
HomoFormer~\cite{xiao2024homoformer} & 39.49 & \textbf{0.993} & \textbf{4.73} & 38.75 & 0.984 & \textbf{2.23} & 35.35 & \textbf{0.975} & \underline{2.64} \\ \hline
\rowcolor[HTML]{DAE8FC} \textbf{PACSRNet (Ours)} & \textbf{40.32} & \textbf{0.993} & \underline{4.89} & \textbf{39.18} & \underline{0.985} & \underline{2.27} & \textbf{36.02} & \underline{0.972} & \textbf{2.63} \\ \hline
\end{tabular}}
\caption{Quantitative comparisons with the SOTA methods on ISTD+ dataset. The best and the second results are \textbf{boldfaced} and \underline{underlined}, respectively.}
\label{tab2}
\end{table*}
